A survey on natural language processing (nlp) and applications in insurance

Text is the most widely used means of communication today. This data is abundant but nevertheless complex to exploit within algorithms. For years, scientists have been trying to implement different techniques that enable computers to replicate some mechanisms of human reading. During the past five years, research disrupted the capacity of the algorithms to unleash the value of text data. It brings today, many opportunities for the insurance industry.Understanding those methods and, above all, knowing how to apply them is a major challenge and key to unleash the value of text data that have been stored for many years. Processing language with computer brings many new opportunities especially in the insurance sector where reports are central in the information used by insurers. SCOR's Data Analytics team has been working on the implementation of innovative tools or products that enable the use of the latest research on text analysis. Understanding text mining techniques in insurance enhances the monitoring of the underwritten risks and many processes that finally benefit policyholders.This article proposes to explain opportunities that Natural Language Processing (NLP) are providing to insurance. It details different methods used today in practice traces back the story of them. We also illustrate the implementation of certain methods using open source libraries and python codes that we have developed to facilitate the use of these techniques.After giving a general overview on the evolution of text mining during the past few years,we share about how to conduct a full study with text mining and share some examples to serve those models into insurance products or services. Finally, we explained in more details every step that composes a Natural Language Processing study to ensure the reader can have a deep understanding on the implementation.

==> dependencies.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{helvet}

%to get Arial-like font but it is quite ugly...
%\renewcommand{\rmdefault}{phv} % Arial
%\renewcommand{\sfdefault}{phv} % Arial

\usepackage[acronym, toc]{glossaries}
\usepackage[round]{natbib} % Natbib setup for author-year style
\usepackage{stmaryrd}
\usepackage[english]{babel}
\usepackage{geometry}
\geometry{a4paper}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{multirow}
\usepackage{url}
\usepackage{xcolor}
\usepackage{color}
\usepackage{setspace}
\usepackage{graphics}
\DeclareGraphicsExtensions{.jpg,.ps,.pdf,.png,.eps}
\usepackage{float}
\usepackage{endnotes}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{lscape}
\usepackage{rotating}
\usepackage{multirow}
%\usepackage{slashbox} %not supported in Shared LaTeX
\usepackage{color}
\usepackage{xcolor}
\usepackage{fancyhdr}
%\pagestyle{fancy}
\usepackage{lastpage}
\usepackage{appendix}
\usepackage{dsfont}
\usepackage{caption}
\usepackage{hhline}
\usepackage{sectsty}
\usepackage{pgf,tikz}
\usepackage{natbib}
\usetikzlibrary{arrows}
\usetikzlibrary{positioning}
\usetikzlibrary{shapes}
\usepackage[capposition=top]{floatrow}
% Fancy headers with scor's blue
\definecolor{scor_blue}{RGB}{0,107,140} %SCOR color
\definecolor{scor_grey}{RGB}{127,127,127} %SCOR color
\chapterfont{\color{scor_blue}}  % sets colour of chapters
\sectionfont{\color{scor_blue}}  % sets colour of sections
\subsectionfont{\color{scor_blue}}  % sets colour of sections
\subsubsectionfont{\color{scor_grey}}  % sets colour of sections
\usepackage{titlesec}
\newcommand{\hsp}{\hspace{20pt}}
\titleformat{\chapter}[hang]{\huge\bfseries\color{scor_blue}}{\thechapter\hsp}{0pt}{\huge}

\usepackage[font={color=scor_blue,bf}]{caption} %figures title in scor blue

%\usepackage{indentfirst}
%\setlength\parindent{0pt} %no paragraph indent
\usepackage[parfill]{parskip}

% All this to save a few trees
\topmargin -1.5cm
\textwidth 14.7cm
\textheight 24cm
\oddsidemargin 0.5cm
\frenchspacing
\onehalfspacing
\headsep 1cm

% Set head and foot
\fancypagestyle{plain}{
    \fancyhf{}% Clear header/footer
    \renewcommand\headrulewidth{0pt}
    \fancyfoot[L]{\includegraphics[scale=0.055]{logos/SCOR_logo.png}}
    \fancyfoot[R]{\textcolor{scor_blue}{\textbf{\thepage}}}
    \renewcommand\footrulewidth{0.5pt}
}
\pagestyle{plain}% Set page style to plain.


%commands to cite
\newcommand{\cay}[1]{[\citeauthor{#1} \citeyear{#1}]}
\newcommand{\cayNP}[1]{\citeauthor{#1} (\citeyear{#1})}

\usepackage{hyperref} 

==> glossary.tex <==
\newglossaryentry{fine-tuned}
{
    name=Fine-tuning,
    description={Is the operation of taking a model that has already been trained once on a specific task, and re-train it on a similar task}
}

\newglossaryentry{semantic}
{
    name=Semantic,
    description={Refers to the study of meanings in a language. It also involves catching all the subtleties of a language in a text}
}

\newglossaryentry{regular expression}
{
    name = Regular expression,
    description={A method of retrieving expressions from a text by looking for a certain pattern. For instance, the regular expression "Mr /. (. *)" allows you to look for all the texts starting with "Mr" and to be interested in the group which follows it which is supposed to represent the name of the person. More precise rules allow to specify the authorized character values with which the pattern is supposed to correspond}
}

\newglossaryentry{statistical learning}
{
    name = Statistical learning,
    description =  {(Taken from \cay{9910207152902121}). Statistical learning refers to a set of tools for modeling and understanding complex datasets. It is a recently developed area in statistics and blends with parallel developments in computer science and, in particular, machine learning. The field encompasses many methods such as [regression and classification] in order to find a predictive function based on data}
}

\newglossaryentry{tokenization}
{
    name = Tokenization,
    description =  {
    1. The action of splitting a text into smaller parts (preprocessing).
    \newline
    2. The action of building a dictionary with the available words and assigning an index of the dictionary to each word (text embedding)}
}

\newglossaryentry{model interpretability}
{
    name = Model Interpretability,
    description =  {When using a model it is important to understand what led it to take a decision. Model interpretability addresses the issue of explaining the predictions made by a model in order to understand if its reasoning is consistent or not}
}

\newglossaryentry{character (maths)}
{
    name = Character (maths),
    description =  {Let $c\in\mathbb{R}^{n}$ be a vector of dimension $n \in \mathbb{N}$ called "character". It could be letter or punctuation or any unitary symbol}
}

\newglossaryentry{segment (maths)}
{
    name = Segment (maths),
    description =  {We define a "segment" $w\in(\mathbb{R}^n)^{\mathbb{N}}$ as a finite sequence of "characters". It could be a word (if the "characters" are letters)}
}

\newglossaryentry{dictionary (maths)}
{
    name = Dictionary (maths),
    description =  {We define a "dictionary" as a subset $\mathcal{D}\subset{(\mathbb{R}^n)^{\mathbb{N}}}$}
}

\newglossaryentry{document (maths)}
{
    name = Document (maths),
    description =  {We define a "document" $d$ $\in\mathcal{D}^{\mathbb{N}}$ as a finite sequence of "segments".
    \begin{center}
        $d = (w_i)_{i \in \llbracket{1,n_d}\rrbracket}$ with $n_d$ the length of the document 
        \end{center}}
}

\newglossaryentry{corpus}
{
    name = Corpus,
    description =  {A set or collection of textual documents.}
}

\newglossaryentry{Neural Network}
{
    name = Neural Network/ Artificial Neural Networks,
    description =  {A type of model using statistical learning designed to reproduce the way human memory functions. Though the main idea is the same as other statistical models, Neural Networks are more complex. During training, weights are adjusted in each neurons. Later on, these weights' values are what allows Neural Networks to operate on unknown data}
}

\newglossaryentry{Training}
{
    name = Training,
    description =  {Training is the part of statistical learning when the model learns how to predict a variable correctly. During this phase, if the model gets a wrong prediction, it will be adjusted toward the right one. After training comes evaluation}
}

\newglossaryentry{Evaluation}
{
    name = Evaluation,
    description =  {Evaluation is the part of statistical learning when the model is tested. At this point, the model is working on data it has not seen during training, allowing to see if the model's performance is consistent or not}
}

\newglossaryentry{Text mining}
{
    name = Text mining,
    description =  {The analysis of textual data and extraction of information from text}
}

\newglossaryentry{Natural Language Processing (NLP)}
{
    name = Natural Language Processing (NLP),
    description =  {The ability for computers to understand human language. It's a field between computer science, text mining and linguistics}
}

\newglossaryentry{Named Entity Recognition (NER)}
{
    name = Named Entity Recognition (NER),
    description =  {gathers all the techniques used to extract from a text the value of a common or proper noun (Organization, location, person, etc.). It also extends to the recognition of metric values (price, date, etc.)}
}

\newglossaryentry{Preprocessing}
{
    name = Preprocessing,
    description =  {Operation of cleaning the data so that it becomes ready to be handled by a model}
}

\newglossaryentry{Text Embedding}
{
    name = Text Embedding,
    description =  {Conversion of textual data into numerical vectors}
}

\newglossaryentry{ Application programming interface (API)}
{
    name = Application programming interface (API),
    description =  {It is the interface between the graphical interface and the provided services. It takes a user request as an entry, applies the service to it and gives the results as an output. The result is then sent to the web graphical interface in order to be communicated to the user}
}

\newglossaryentry{Web Graphical Interface}
{
    name = Web graphical interface,
    description =  {It is the interface between the user and the API. It puts everything that is given by the API into a presentable form for the user and translates the requests from the user into a language that is understood by the API}
}

\newglossaryentry{Attention}
{
    name = Attention,
    description =  {Attention is a mechanism that that draws the relationships between the elements of a sequence. In other words, this mechanism emphasizes how every part of an input interact between themselves and how much influence one part has on another one. These interactions, which reproduce the context of the input, are represented in an Attention Matrix. This mechanism aims to reproduce the way the human brain connects each words of a sentence with the others when reading, while saving time and resources because it allows to focus the calculations on the relevant parts of a sequence. Attention model, Attention mechanism and Attention matrix refers to the same concept}
}

\newglossaryentry{Transformers Neural Networks}
{
    name = Transformers Neural Networks,
    description =  {A type of neural networks that mainly combines Attention with Feedforward Neural Networks. It's great advantage is that it is less complex and faster compared to RNN on similar tasks}
}

\newglossaryentry{Feedforward Neural Networks}
{
    name = Feedforward Neural Networks,
    description =  {The simplest type of neural networks there is, where information only circulates in one direction from a single entry to a single prediction, unlike RNN where information can be kept and used for several predictions}
}

\newglossaryentry{Recurrent Neural Networks (RNN)}
{
    name = Recurrent Neural Networks (RNN),
    description =  { A type of neural networks that has access to past predictions when making a new prediction. The information about previous outputs is conveyed through "hidden states". RNN are able to work on sequential problems, which are problems that involve sequences of different sizes, such as translation. An article from \cite{RNN} explains the concept of RNN with further details, and a cheat sheet from \cite{CS230} summarizing the mathematical background around RNN is available on Stanford University's website }
}

\newglossaryentry{Encoder-Decoder}
{
    name = Encoder-Decoder,
    description =  { Also called Sequence-to-Sequence (Seq2Seq), an architecture using RNNs introduced by \cayNP{sutskever2014sequence}. It performs well when the input's and output's lengths differ. An article from \cite{encoderdecoder} explains how the encoder-decoder architecture is built and how it allows better performances}
}

\newglossaryentry{Bidirectional Encoder Representation for Transformers (BERT)}
{
    name = Bidirectional Encoder Representation for Transformers (BERT),
    description =  {A deep neural networks based model which consists of a succession of encoders extracted from Transformers Neural Networks. This type of model proved to achieve solid results on NLP tasks although they hare very complex and take long to be calibrated}
}

